On the Upward/Downward Closures of Petri Nets

We study the size and the complexity of computing finite state automata (FSA) representing and approximating the downward and the upward closure of Petri net languages with coverability as the acceptance condition. We show how to construct an FSA recognizing the upward closure of a Petri net language in doubly-exponential time, and therefore the size is at most doubly exponential. For downward closures, we prove that the size of the minimal automata can be non-primitive recursive. In the case of BPP nets, a well-known subclass of Petri nets, we show that an FSA accepting the downward/upward closure can be constructed in exponential time. Furthermore, we consider the problem of checking whether a simple regular language is included in the downward/upward closure of a Petri net/BPP net language. We show that this problem is EXPSPACE-complete (resp. NP-complete) in the case of Petri nets (resp. BPP nets). Finally, we show that it is decidable whether a Petri net language is upward/downward closed. To this end, we prove that one can decide whether a given regular language is a subset of a Petri net coverability language.

==> content/prelims.tex <==
%!TEX root = ../PetriClosures.tex

\section{Preliminaries}
\label{Section:Preliminaries}

We recall the basic notions concerning Petri nets and language closures following standard textbooks~\cite{Reisig1985}.
A \emph{(labeled) Petri net} is a tuple \mbox{$N = (\Sigma,P,T,F,\lambda)$}.
Here, $\Sigma$ is a finite alphabet, $P$ a finite set of \emph{places}, $T$ a finite set of \emph{transitions}, $F: (P \times T) \cup (T \times P) \rightarrow \N$ a \emph{flow function}, and $\lambda: T \mapsto \Sigma\cup\set{\varepsilon}$ is a labeling function with $\varepsilon$ being the empty word.
When convenient, we will assume that the places are ordered, \ie $P = \oneto{\ell}$ for some $\ell \in \N$.
For any place or transition $x \in P \cup T$, we define the \emph{preset} to consist of the elements that have an arc to the corresponding place or transition, $\Pred{x} = \Set{ y \in P \cup T}{ F(y,x) > 0 }$.
The \emph{postset} is defined similarly,
$\Succ{x} = \Set{ y \in P \cup T }{ F(x,y) > 0 }$. 

To define the semantics of Petri nets, we use \emph{markings} $M: P \rightarrow \N$, runtime configurations that assign to each place a number of \emph{tokens}.
A marking $M$ \emph{enables} a transition $t$, denoted $\TJustEnable {M} {t}$, if \mbox{$M(p) \geq F(p,t)$} for all $p \in P$.
A transition $t$ that is enabled may be \emph{fired}, leading to the new marking $M'$ defined by $M'(p) = M(p) - F(p,t) + F(t,p)$ for all $p \in P$, \ie $t$~consumes $F(p,t)$ many tokens and produces $F(t,p)$ many tokens in $p$.
We write the firing relation as $\TEnable {M} {t} {M'}$.
A \emph{computation} \mbox{$\pi = M_0 \move{t_1} M_1 \cdots \move{t_m} M_m$} consists of markings and transitions.
We extend the firing relation to transition sequences $\sigma=t_1\ldots t_m$ and also write $\pi = M_0\move{\sigma} M_m$. 
%The \emph{length} of $\pi$ is the number of transitions, $m$.
A marking $M$ is \emph{reachable} from an initial marking $M_0$ if $\TEnable {M_0}{\sigma} {M}$ for some $\sigma\in T^*$
%We write $R(M_0)$ to denote the set of all reachable markings from a given initial marking $M_0$. 
A marking $M$ covers another marking $M_f$, denoted $M \geq M_f$, if $M(p) \geq M_f(p)$ for all $p \in P$.
A marking $M_f$ is \emph{coverable} from $M_0$ if there is a marking $M$ reachable from $M_0$ that covers $M_f$, $\TEnable{M_0}{\sigma}{M}\geq M_f$ for some $\sigma\in T^*$.

Given a Petri net $N$, an initial marking $M_0$, and a final marking $M_f$,
%to be covered,
the associated \emph{covering language} is
\[
    L(N,M_0,M_f) = \Set{ \lambda(\sigma)}{\sigma \in T^*,\  \TEnable{M_0}{\sigma}{M}\geq M_f }
    \ .  
\]
Given a natural number $k \in \N$, we define
\[
    L_k(N,M_0,M_f) = \Set{ \lambda(\sigma)}{\sigma \in T^{\leq k},\ \TEnable{M_0}{\sigma}{M}\geq M_f }
\]
to be the set of words accepted by computations of length at most $k$.

When we refer to the \emph{size} of a Petri net or a marking, denoted $\card{N}$ and $\card{M}$, respectively, we assume the token counts and the arc weights to be encoded in binary (with $0$ needing one bit) and sum up all numbers.
Thus, $\card{N}=O(|P| \cdot |T|)$. 

We define the \emph{token count} $\tokencount{M}$ of a marking $M$ to be the sum of all tokens assigned by $M$, $\tokencount{M} = \Sigma_{p\in P}M(p)$.

A Petri net $N$ is said to be a \emph{BPP net} if every transition consumes at most one from one place (\ie $\Sigma_{p\in P}F(p, t)\leq 1$ for every $t \in T$).




\begin{lemma}
\label{k-boundedlanguages}
    Consider $N, M_0,$ and $M_f$
    For every $k \in \N$, we can construct a finite automaton of size  $O( (k+2)^{\poly({n})})$ that  accepts $L_k(N,M_0,M_f)$, where $n = \card{N} + \card{M_0} + \card{M_f}$.
\end{lemma}

The closures we study are defined \wrt the \emph{subword relation} $\subword\ \, \subseteq \Sigma^*\!\times\Sigma^*$ \cite{Higman52}. 
A word $u = a_1 \ldots a_n$ is a subword of $v$, denoted $u \subword v$, if $u$ can be obtained by deleting letters from $v$ or, equivalently, if $v = v_0 a_1 v_1 \ldots a_n v_{n}$ for some \mbox{$v_0, \ldots, v_{n} \in \Sigma^*$.}
The \emph{upward closure} of \mbox{$L\subseteq \Sigma^*$} consists of all words that have a subword in the language,
\mbox{$\uc{L} = \Set{v\in\Sigma^*}{\exists u \in L: u \subword v}$.}
The \emph{downward closure} of $L$ contains all words that are dominated by a word in the language, 
\mbox{$\dc{L} = \Set{ u\in\Sigma^* }{\exists v \in L: u \subword v}$.}
Higman showed that the subword relation is a well-quasi-ordering~\cite{Higman52}, which means that every set of words $S\subseteq \Sigma^*$ has a finite \emph{basis} --- a finite set of \emph{minimal elements} $v\in S$ such that $\nexists u\in S: u\subword v$.
With finite bases, $\uc{L}$ and $\dc{L}$ are guaranteed to be regular for every language $L\subseteq \Sigma^*$~\cite{Haines1969}. 
Indeed, they can be expressed using  the subclass of simple regular languages defined by so-called \emph{simple regular expressions}~\cite{Bouajjani2004}. 
These SREs are choices among \emph{products} $\product$, which in turn interleave single letters $a$ or $(a+\varepsilon)$ with iterations over letters from subsets $\Gamma\subseteq \Sigma$ of the alphabet:
%
\begin{align*}
    \sre&::=\product\bnf\sre+\sre
    &\product&::=a \bnf (a+\varepsilon)\bnf\Gamma^*\bnf\product.\product\ .
\end{align*}

The \emph{Parikh image} of a word~\cite{Parikh1966} counts the number of occurrences of all letters while forgetting about their relative positioning.
Formally, the function $\Parikh : \Sigma^* \mapsto \N^{\Sigma}$ takes a word $w\in\Sigma^*$ and gives the function $\Parikh(w):\Sigma\rightarrow\N$ defined by $(\Parikh(w))(a) =\card{\Prj{w}{\{a\}}}$ for all $a\in \Sigma$.
Here, $\Prj{w}{\Gamma}$ is the projection of the word $w$ onto the letters from the subalphabet $\Gamma\subseteq \Sigma$.
Moreover, $\card{w}$ is the length of a word, with $\card{\varepsilon}=0$.


==> style/abbrev_de.tex <==
% ######################
% ABBREVIATIONS
% ######################

% small
\newcommand{\bzgl}
{bzgl.~}

\newcommand{\obda}
{o.B.d.A.~}

\newcommand{\bzw}
{bzw.~}

\newcommand{\zb}
{z.B.~}

% capital
\newcommand{\Obda}
{O.B.d.A.~}

\newcommand{\Zb}
{Z.B.~}


==> style/abbrev_en.tex <==
% ######################
% ABBREVIATIONS
% ######################

% small
\newcommand{\wrt}
{wrt.~}

\newcommand{\ie}
{i.e.~}

\newcommand{\eg}
{e.g.~}

\newcommand{\resp}
{resp.~}

\newcommand{\sth}
{s.t.~}

\newcommand{\wolog}
{wlog.~}

% capital
\newcommand{\Ie}
{I.e.~}

\newcommand{\Eg}
{E.g.~}

\newcommand{\Wolog}
{Wlog.~}


==> style/algo.tex <==
% ############
% ALGORITHMS
% ############

% algorithms
\usepackage{algorithmicx}
\usepackage{algpseudocode}

%
% begin vertical rule patch for algorithmicx (http://tex.stackexchange.com/questions/144840/vertical-loop-block-lines-in-algorithmicx-with-noend-option)
%

% note that some of the packages above are also needed
\newcommand{\ALGtikzmarkcolor}{black}% customise this, if you want
\newcommand{\ALGtikzmarkextraindent}{4pt}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetstart}{-.5ex}% customise this, if you want
\newcommand{\ALGtikzmarkverticaloffsetend}{-.5ex}% customise this, if you want
\makeatletter
\newcounter{ALG@tikzmark@tempcnta}

\newcommand\ALG@tikzmark@start{%
    \global\let\ALG@tikzmark@last\ALG@tikzmark@starttext%
    \expandafter\edef\csname ALG@tikzmark@\theALG@nested\endcsname{\theALG@tikzmark@tempcnta}%
    \tikzmark{ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname}%
    \addtocounter{ALG@tikzmark@tempcnta}{1}%
}

\def\ALG@tikzmark@starttext{start}
\newcommand\ALG@tikzmark@end{%
    \ifx\ALG@tikzmark@last\ALG@tikzmark@starttext
    % ignore this, the block was opened then closed directly without any other blocks in between (so just a \State basically)
    % don't draw a vertical line here
    \else
    \tikzmark{ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname}%
    \tikz[overlay,remember picture] \draw[\ALGtikzmarkcolor] let \p{S}=($(pic cs:ALG@tikzmark@start@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetstart)$), \p{E}=($(pic cs:ALG@tikzmark@end@\csname ALG@tikzmark@\theALG@nested\endcsname)+(\ALGtikzmarkextraindent,\ALGtikzmarkverticaloffsetend)$) in (\x{S},\y{S})--(\x{S},\y{E});%
    \fi
    \gdef\ALG@tikzmark@last{end}%
}
% the following line injects our new tikzmarking code
\apptocmd{\ALG@beginblock}{\ALG@tikzmark@start}{}{\errmessage{failed to patch}}
\pretocmd{\ALG@endblock}{\ALG@tikzmark@end}{}{\errmessage{failed to patch}}
\makeatother

%
% end vertical rule patch for algorithmicx
%

\let\Cmd\State

% C-style comments
\renewcommand {\algorithmiccomment}[1]
    {\hfill $/ \!/$ #1}
   
% return on new line
\let\oldReturn\Return
\renewcommand{\Return}{\Cmd\oldReturn}

% commands like in algorith2e
\newcommand {\ForLoop} [2]
{
    \For {#1}
        #2
    \EndFor
}

\newcommand {\WhileLoop} [2]
{
    \While {#1}
        #2
    \EndWhile
}

\newcommand {\IfCond} [2]
{
    \If {#1}
        #2
    \EndIf
}

\newcommand {\IfElseCond} [3]
{
    \If {#1}
        #2
    \Else
        #3
    \EndIf
}


==> style/article.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

%
% Bibliography & references
%

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,maxbibnames=9,maxcitenames=9,backend=bibtex,giveninits=true,isbn=false,doi=false]{biblatex}
\DeclareFieldFormat*{title}{\mkbibitalic{#1\isdot}}
\DeclareFieldFormat*{booktitle}{#1\isdot}
\DeclareFieldFormat*{journaltitle}{#1\isdot}
%\DeclareFieldFormat{titlecase}{\MakeSentenceCase{#1}}
%\newbibmacro*{journal}{%
%    \iffieldundef{journaltitle}
%    {}
%    {\printtext[journaltitle]{%
%            \printfield[noformat]{journaltitle}%
%            \setunit{\subtitlepunct}%
%            \printfield[noformat]{journalsubtitle}}}}

%
% Includes
%

% underlining
\usepackage{ulem}
% set emph back to normal (instead of underlined)
\normalem 

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

%
% TOC and hyperlinks
%
\PassOptionsToPackage{obeyspaces}{url}
\usepackage[bookmarksnumbered]{hyperref} 

% fix nesting in PDF TOC
\usepackage[open=true]{bookmark}


% don't show subsections in TOC
\setcounter{tocdepth}{1}

%
% emph as bold
%

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother
\newcommand{\aemph}[1]{\textit{#1}}


%
% Clever references
%

% clever references
\usepackage{cleveref}
% use capital references by default
\let\scref\cref
\let\cref\Cref


%
% Page layout
%
\usepackage[]{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot=1cm}

\usepackage[headsepline]{scrlayer-scrpage}
%\clearpairofpagestyles
\clearscrheadfoot
\ihead{\normalfont \headmark}
\cfoot{\Large \pagemark}
\automark[]{section}

% space between lines
\onehalfspacing

%
% Hyphenation & separation
%
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%
% Redefined environment
%

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% shortproof without newline
\makeatletter
\newenvironment{shortproof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother


%
% Theorem styles
%

% Theorem numbering
\def\theoremnumberstyle{changesection}

% Theoremstyle
\newtheoremstyle{withnumber} % name
{0.4cm}                      % Space above
{0.6cm}                      % Space below
{\normalfont}                % Body font
{}                           % Indent amount
{\bfseries}                  % Theorem head font
{\newline}                   % Punctuation after theorem head
{0.2cm}                      % Space after theorem head
{#2 #1\thmnote{: \ #3}}      % Theorem head spec (can be left empty, meaning ‘normal’)

\newtheoremstyle{nonumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}              % Body font
{}                         % Indent amount
{\bfseries}                % Theorem head font
{\newline}                 % Punctuation after theorem head
{0.2cm}                    % Space after theorem head
{#1\thmnote{: \ #3}}       % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{withnumber} 

%
% Hackfix for itemize / enumerate at the beginning of a theorem
%
\newcommand{\skipfix}{\leavevmode\vspace{-2.2em}}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \skipfix
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \skipfix
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
%\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
%\usepackage{capt-of}
%\usepackage{caption}
%\DeclareCaptionFont{white}{\color{white}}
%\DeclareCaptionFormat{listing}
%{
%    \colorbox[cmyk]{1, 1, 1,0.01}
%    {
%        \parbox{\textwidth}
%        {\hspace{15pt}#1#2#3}
%    }
%}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
%\usepackage{listings}
%\lstset{
%    numbers=left,
%    numberstyle=\tiny,
%    numbersep=5pt,
%    keywordstyle=\color{black}\bfseries,
%    stringstyle=\ttfamily,
%    showstringspaces=false,
%    basicstyle=\footnotesize,
%    captionpos=b
%}
%\lstset{language=java}
%% Listings
%\lstset{
%    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
%    numbers=left,               % Ort der Zeilennummern
%    numberstyle=\tiny,          % Stil der Zeilennummern
%    %stepnumber=2,               % Abstand zwischen den Zeilennummern
%    numbersep=5pt,              % Abstand der Nummern zum Text
%    tabsize=4,                  % Groesse von Tabs
%    extendedchars=true,         %
%    breaklines=true,            % Zeilen werden Umgebrochen
%    keywordstyle=\text,
%    %frame=b,         
%    stringstyle=\color{black}\ttfamily, % Farbe der String
%    showspaces=false,           % Leerzeichen anzeigen ?
%    showtabs=false,             % Tabs anzeigen ?
%    xleftmargin=5pt,
%    framexleftmargin=17pt,
%    framexrightmargin=5pt,
%    framexbottommargin=4pt,
%    %backgroundcolor=\color{lightgray},
%    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
%    captionpos=t,     
%}
%\lstloadlanguages{% Check Dokumentation for further languages ...
%    %[Visual]Basic
%    %Pascal
%    %C
%    %C++
%    %XML
%    %HTML
%    Java
%}

%
% Colors
%

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}

%
% Boxes for computational problems
%

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
%    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/commands.tex <==
% ##########
% COMMANDS
% ##########

% custom emph
\providecommand {\aemph}[1]
{\textbf{#1}}

% bold + italic
\newcommand {\textbfit} [1]
{\textbf{\textit{#1}}}

% monospace (+ bold & italic)
\newcommand {\mono} [1]
{\texttt{#1}}

\newcommand {\monobf} [1]
{\texttt{\bfseries #1}}

\newcommand {\monobfit} [1]
{\texttt{\bfseries \itshape #1}}

\newcommand {\monoit} [1]
{\texttt{\itshape #1}}

% blackboard bold letters
\providecommand\A{}
\renewcommand {\A} {{\mathbb A}}
\providecommand\B{}
\renewcommand {\B} {{\mathbb B}}
\providecommand{\C}{}
\renewcommand {\C} {{\mathbb C}}
\providecommand\D{}
\renewcommand {\D} {{\mathbb D}}
\providecommand\E{}
\renewcommand {\E} {{\mathbb E}}
\providecommand\F{}
\renewcommand {\F} {{\mathbb F}}
\providecommand {\G} {}
\renewcommand {\G} {{\mathbb G}}
\providecommand\H{}
\renewcommand {\H} {{\mathbb H}}
\providecommand\I{}
\renewcommand {\I} {{\mathbb I}}
\providecommand\J{}
\renewcommand {\J} {{\mathbb J}}
\providecommand\K{}
\renewcommand {\K} {{\mathbb K}}
\providecommand\K{}
\renewcommand {\L} {{\mathbb L}}
\providecommand {\M} {}
\renewcommand {\M} {{\mathbb M}}
\providecommand\N{}
\renewcommand {\N} {{\mathbb N}}
\providecommand\O{}
\renewcommand {\O} {{\mathbb O}}
\providecommand\P{}
\renewcommand {\P} {{\mathbb P}}
\providecommand\Q{}
\renewcommand {\Q} {{\mathbb Q}}
\providecommand\R{}
\renewcommand {\R} {{\mathbb R}}
\providecommand\S{}
\renewcommand {\S} {{\mathbb S}}
\providecommand {\T} {}
\renewcommand {\T} {{\mathbb T}}
\providecommand{\U}{}
\renewcommand {\U} {{\mathbb U}}
\providecommand\V{}
\renewcommand {\V} {{\mathbb V}}
\providecommand\W{}
\renewcommand {\W} {{\mathbb W}}
\providecommand\X{}
\renewcommand {\X} {{\mathbb X}}
\providecommand\Y{}
\renewcommand {\Y} {{\mathbb Y}}
\providecommand\Z{}
\renewcommand {\Z} {{\mathbb Z}}

% calligraphic letters
\newcommand {\calA} {\mathcal{A}}
\newcommand {\calB} {\mathcal{B}}
\newcommand {\calC} {\mathcal{C}}
\newcommand {\calD} {\mathcal{D}}
\newcommand {\calE} {\mathcal{E}}
\newcommand {\calF} {\mathcal{F}}
\newcommand {\calG} {\mathcal{G}}
\newcommand {\calH} {\mathcal{H}}
\newcommand {\calI} {\mathcal{I}}
\newcommand {\calJ} {\mathcal{J}}
\newcommand {\calK} {\mathcal{K}}
\newcommand {\calL} {\mathcal{L}}
\newcommand {\calM} {\mathcal{M}}
\newcommand {\calN} {\mathcal{N}}
\newcommand {\calO} {\mathcal{O}}
\newcommand {\calP} {\mathcal{P}}
\newcommand {\calQ} {\mathcal{Q}}
\newcommand {\calR} {\mathcal{R}}
\newcommand {\calS} {\mathcal{S}}
\newcommand {\calT} {\mathcal{T}}
\newcommand {\calU} {\mathcal{U}}
\newcommand {\calV} {\mathcal{V}}
\newcommand {\calW} {\mathcal{W}}
\newcommand {\calX} {\mathcal{X}}
\newcommand {\calY} {\mathcal{Y}}
\newcommand {\calZ} {\mathcal{Z}}
\newcommand {\cala} {\mathcal{a}}
\newcommand {\calb} {\mathcal{b}}
\newcommand {\calc} {\mathcal{c}}
\newcommand {\cald} {\mathcal{d}}
\newcommand {\cale} {\mathcal{e}}
\newcommand {\calf} {\mathcal{f}}
\newcommand {\calg} {\mathcal{g}}
\newcommand {\calh} {\mathcal{h}}
\newcommand {\cali} {\mathcal{i}}
\newcommand {\calj} {\mathcal{j}}
\newcommand {\calk} {\mathcal{k}}
\newcommand {\call} {\mathcal{l}}
\newcommand {\calm} {\mathcal{m}}
\newcommand {\caln} {\mathcal{n}}
\newcommand {\calo} {\mathcal{o}}
\newcommand {\calp} {\mathcal{p}}
\newcommand {\calq} {\mathcal{q}}
\newcommand {\calr} {\mathcal{r}}
\newcommand {\cals} {\mathcal{s}}
\newcommand {\calt} {\mathcal{t}}
\newcommand {\calu} {\mathcal{u}}
\newcommand {\calv} {\mathcal{v}}
\newcommand {\calw} {\mathcal{w}}
\newcommand {\calx} {\mathcal{x}}
\newcommand {\caly} {\mathcal{y}}
\newcommand {\calz} {\mathcal{z}}

% blackboard bold letters
\newcommand {\bbA} {\mathbb{A}}
\newcommand {\bbB} {\mathbb{B}}
\newcommand {\bbC} {\mathbb{C}}
\newcommand {\bbD} {\mathbb{D}}
\newcommand {\bbE} {\mathbb{E}}
\newcommand {\bbF} {\mathbb{F}}
\newcommand {\bbG} {\mathbb{G}}
\newcommand {\bbH} {\mathbb{H}}
\newcommand {\bbI} {\mathbb{I}}
\newcommand {\bbJ} {\mathbb{J}}
\newcommand {\bbK} {\mathbb{K}}
\newcommand {\bbL} {\mathbb{L}}
\newcommand {\bbM} {\mathbb{M}}
\newcommand {\bbN} {\mathbb{N}}
\newcommand {\bbO} {\mathbb{O}}
\newcommand {\bbP} {\mathbb{P}}
\newcommand {\bbQ} {\mathbb{Q}}
\newcommand {\bbR} {\mathbb{R}}
\newcommand {\bbS} {\mathbb{S}}
\newcommand {\bbT} {\mathbb{T}}
\newcommand {\bbU} {\mathbb{U}}
\newcommand {\bbV} {\mathbb{V}}
\newcommand {\bbW} {\mathbb{W}}
\newcommand {\bbX} {\mathbb{X}}
\newcommand {\bbY} {\mathbb{Y}}
\newcommand {\bbZ} {\mathbb{Z}}
\newcommand {\bba} {\mathbb{a}}
\newcommand {\bbb} {\mathbb{b}}
\newcommand {\bbc} {\mathbb{c}}
\newcommand {\bbd} {\mathbb{d}}
\newcommand {\bbe} {\mathbb{e}}
\newcommand {\bbf} {\mathbb{f}}
\newcommand {\bbg} {\mathbb{g}}
\newcommand {\bbh} {\mathbb{h}}
\newcommand {\bbi} {\mathbb{i}}
\newcommand {\bbj} {\mathbb{j}}
\newcommand {\bbk} {\mathbb{k}}
\newcommand {\bbl} {\mathbb{l}}
\newcommand {\bbm} {\mathbb{m}}
\newcommand {\bbn} {\mathbb{n}}
\newcommand {\bbo} {\mathbb{o}}
\newcommand {\bbp} {\mathbb{p}}
\newcommand {\bbq} {\mathbb{q}}
\newcommand {\bbr} {\mathbb{r}}
\newcommand {\bbs} {\mathbb{s}}
\newcommand {\bbt} {\mathbb{t}}
\newcommand {\bbu} {\mathbb{u}}
\newcommand {\bbv} {\mathbb{v}}
\newcommand {\bbw} {\mathbb{w}}
\newcommand {\bbx} {\mathbb{x}}
\newcommand {\bby} {\mathbb{y}}
\newcommand {\bbz} {\mathbb{z}}

% letters in Fraktur
\newcommand {\frakA} {\mathfrak{A}}
\newcommand {\frakB} {\mathfrak{B}}
\newcommand {\frakC} {\mathfrak{C}}
\newcommand {\frakD} {\mathfrak{D}}
\newcommand {\frakE} {\mathfrak{E}}
\newcommand {\frakF} {\mathfrak{F}}
\newcommand {\frakG} {\mathfrak{G}}
\newcommand {\frakH} {\mathfrak{H}}
\newcommand {\frakI} {\mathfrak{I}}
\newcommand {\frakJ} {\mathfrak{J}}
\newcommand {\frakK} {\mathfrak{K}}
\newcommand {\frakL} {\mathfrak{L}}
\newcommand {\frakM} {\mathfrak{M}}
\newcommand {\frakN} {\mathfrak{N}}
\newcommand {\frakO} {\mathfrak{O}}
\newcommand {\frakP} {\mathfrak{P}}
\newcommand {\frakQ} {\mathfrak{Q}}
\newcommand {\frakR} {\mathfrak{R}}
\newcommand {\frakS} {\mathfrak{S}}
\newcommand {\frakT} {\mathfrak{T}}
\newcommand {\frakU} {\mathfrak{U}}
\newcommand {\frakV} {\mathfrak{V}}
\newcommand {\frakW} {\mathfrak{W}}
\newcommand {\frakX} {\mathfrak{X}}
\newcommand {\frakY} {\mathfrak{Y}}
\newcommand {\frakZ} {\mathfrak{Z}}
\newcommand {\fraka} {\mathfrak{a}}
\newcommand {\frakb} {\mathfrak{b}}
\newcommand {\frakc} {\mathfrak{c}}
\newcommand {\frakd} {\mathfrak{d}}
\newcommand {\frake} {\mathfrak{e}}
\newcommand {\frakf} {\mathfrak{f}}
\newcommand {\frakg} {\mathfrak{g}}
\newcommand {\frakh} {\mathfrak{h}}
\newcommand {\fraki} {\mathfrak{i}}
\newcommand {\frakj} {\mathfrak{j}}
\newcommand {\frakk} {\mathfrak{k}}
\newcommand {\frakl} {\mathfrak{l}}
\newcommand {\frakm} {\mathfrak{m}}
\newcommand {\frakn} {\mathfrak{n}}
\newcommand {\frako} {\mathfrak{o}}
\newcommand {\frakp} {\mathfrak{p}}
\newcommand {\frakq} {\mathfrak{q}}
\newcommand {\frakr} {\mathfrak{r}}
\newcommand {\fraks} {\mathfrak{s}}
\newcommand {\frakt} {\mathfrak{t}}
\newcommand {\fraku} {\mathfrak{u}}
\newcommand {\frakv} {\mathfrak{v}}
\newcommand {\frakw} {\mathfrak{w}}
\newcommand {\frakx} {\mathfrak{x}}
\newcommand {\fraky} {\mathfrak{y}}
\newcommand {\frakz} {\mathfrak{z}}

% script letters
\newcommand {\scrA} {\mathscr{A}}
\newcommand {\scrB} {\mathscr{B}}
\newcommand {\scrC} {\mathscr{C}}
\newcommand {\scrD} {\mathscr{D}}
\newcommand {\scrE} {\mathscr{E}}
\newcommand {\scrF} {\mathscr{F}}
\newcommand {\scrG} {\mathscr{G}}
\newcommand {\scrH} {\mathscr{H}}
\newcommand {\scrI} {\mathscr{I}}
\newcommand {\scrJ} {\mathscr{J}}
\newcommand {\scrK} {\mathscr{K}}
\newcommand {\scrL} {\mathscr{L}}
\newcommand {\scrM} {\mathscr{M}}
\newcommand {\scrN} {\mathscr{N}}
\newcommand {\scrO} {\mathscr{O}}
\newcommand {\scrP} {\mathscr{P}}
\newcommand {\scrQ} {\mathscr{Q}}
\newcommand {\scrR} {\mathscr{R}}
\newcommand {\scrS} {\mathscr{S}}
\newcommand {\scrT} {\mathscr{T}}
\newcommand {\scrU} {\mathscr{U}}
\newcommand {\scrV} {\mathscr{V}}
\newcommand {\scrW} {\mathscr{W}}
\newcommand {\scrX} {\mathscr{X}}
\newcommand {\scrY} {\mathscr{Y}}
\newcommand {\scrZ} {\mathscr{Z}}
\newcommand {\scra} {\mathscr{a}}
\newcommand {\scrb} {\mathscr{b}}
\newcommand {\scrc} {\mathscr{c}}
\newcommand {\scrd} {\mathscr{d}}
\newcommand {\scre} {\mathscr{e}}
\newcommand {\scrf} {\mathscr{f}}
\newcommand {\scrg} {\mathscr{g}}
\newcommand {\scrh} {\mathscr{h}}
\newcommand {\scri} {\mathscr{i}}
\newcommand {\scrj} {\mathscr{j}}
\newcommand {\scrk} {\mathscr{k}}
\newcommand {\scrl} {\mathscr{l}}
\newcommand {\scrm} {\mathscr{m}}
\newcommand {\scrn} {\mathscr{n}}
\newcommand {\scro} {\mathscr{o}}
\newcommand {\scrp} {\mathscr{p}}
\newcommand {\scrq} {\mathscr{q}}
\newcommand {\scrr} {\mathscr{r}}
\newcommand {\scrs} {\mathscr{s}}
\newcommand {\scrt} {\mathscr{t}}
\newcommand {\scru} {\mathscr{u}}
\newcommand {\scrv} {\mathscr{v}}
\newcommand {\scrw} {\mathscr{w}}
\newcommand {\scrx} {\mathscr{x}}
\newcommand {\scry} {\mathscr{y}}
\newcommand {\scrz} {\mathscr{z}}

% fake capital Greek letters for the sake of complenetess
% upright (instead of italic/slanted) to match the other Greek capitals
%\providecommand{\Alpha} {}
%\renewcommand {\Alpha} {\mathsf{A}}
%\providecommand{\Beta} {}
%\renewcommand {\Beta} {\mathsf{B}}
%\providecommand{\Epsilon} {}
%\renewcommand {\Epsilon} {\mathsf{E}}
%\providecommand{\Zeta} {}
%\renewcommand {\Zeta} {\mathsf{Z}}
%\providecommand{\Eta} {}
%\renewcommand {\Eta} {\mathsf{H}}
%\providecommand{\Iota} {}
%\renewcommand {\Iota} {\mathsf{I}}
%\providecommand{\Kappa} {}
%\renewcommand {\Kappa} {\mathsf{K}}
%\providecommand{\Mu} {}
%\renewcommand {\Mu} {\mathsf{M}}
%\providecommand{\Tau} {}
%\renewcommand {\Tau} {\mathsf{T}}
%\providecommand{\Chi} {}
%\renewcommand {\Chi} {\mathsf{X}}


==> style/definitions.tex <==
% ##################
% DEFINITIONS
% ##################

%
% Basic stuff
%

\newcommand { \from }
{ \leftarrow }

\newcommand {\Rplus} 
{ \R_{>0} }

\newcommand {\true}
{\mathit{true}}

\newcommand {\false}
{\mathit{false}}

\newcommand {\monotrue}
{\mathtt{true}}

\newcommand {\monofalse}
{\mathtt{false}}

\newcommand {\ifalse}
{\mathit{false}}

\newcommand {\itrue}
{\mathit{true}}

\newcommand {\oneto} [1]
{\left\{ 1, \ldots, #1\right\}}

\newcommand {\zeroto} [1]
{\left\{ 0, \ldots, #1\right\}}

\newcommand {\arity} [1]
{ {\scriptstyle / #1 } }

% small @
\newcommand {\at}
{
    \raisebox{0.5mm}{\scalebox{0.7}[0.7]{@}}
}

% corresponds to
\newcommand\corrto{%
    \let\savearraystretch\arraystretch
    \renewcommand\arraystretch{0.3}
    \begin{array}{c}
        \stretchto{
            \scalerel*[\widthof{=}]{\wedge}
            {\rule{1ex}{3ex}}%
        }{0.5ex}\\ 
        =%
    \end{array}
    \let\arraystretch\savearraystretch
}

% stacked logical operators
\newcommand{\wedgevee}
{
    \mathrel{\substack{\wedge\\\vee}}
}
\newcommand{\veewedge}
{
    \mathrel{\substack{\vee\\\wedge}}
}

% small mid for (E)BNF
\newcommand{\bnf}
{\:\shortmid\:}

%
% Sets
%

\newcommand{\card}[1]
{\left|#1\right|}

\newcommand {\set} [1]
{ \left\{ #1 \right\} }

\newcommand {\Set} [2]
{ \left\{ #1 \ \middle| \ #2 \right\} }

\newcommand {\smallset} [2]
{ \{ #1 \mid #2 \} }

\newcommand {\ideal} [1]
{ \langle \ #1 \ \rangle}

\newcommand {\Ideal} [2]
{ \langle \ #1 \mid #2 \ \rangle}

\newcommand {\pwrset} [1]
{ {\mathcal P} \left( #1 \right)}

%
% Set operations
%

% disjoint union
\makeatletter
\providecommand*{\bigdotcup}{%
    \mathbin{%
        \mathpalette\@bigdotcup{}%
    }%
}
\newcommand*{\@bigdotcup}[2]{%
    \ooalign{%
        $\m@th#1\bigcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\providecommand*{\dotcup}{%
    \mathbin{%
        \mathpalette\@dotcup{}%
    }%
}
\newcommand*{\@dotcup}[2]{%
    \ooalign{%
        $\m@th#1\cup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\providecommand*{\bigdotsqcup}{%
    \mathbin{%
        \mathpalette\@bigdotsqcup{}%
    }%
}
\newcommand*{\@bigdotsqcup}[2]{%
    \ooalign{%
        $\m@th#1\bigsqcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\providecommand*{\dotsqcup}{%
    \mathbin{%
        \mathpalette\@dotsqcup{}%
    }%
}
\newcommand*{\@dotsqcup}[2]{%
    \ooalign{%
        $\m@th#1\sqcup$\cr
        \hidewidth$\m@th#1\cdot$\hidewidth
    }%
}
\makeatother

%
% Closures
%

\newcommand{\up}
{\!\uparrow}

\newcommand{\down}
{\!\downarrow}

\newcommand{\dc}[1]
{#1\down }

\newcommand{\uc}[1]
{#1\up }

%
% Logic
%

% semantic brackets
\newcommand {\sem}[1]
{	\left\llbracket #1 \right\rrbracket }

% inverse models
\makeatletter
\providecommand*{\Dashv}{%
    \mathrel{%
        \mathpalette\@Dashv\vDash
    }%
}
\makeatother

% logical equivalence (\models \ismod)
\newcommand{\lequiv}{\vDash\hspace{-2pt}\Dashv}

%
% Complexity
%

\newcommand {\bigO} [1]
{ \calO \left( {#1} \right) }

\newcommand {\smallO} [1]
{ o \left( #1 \right) }

\newcommand {\bigOmega} [1]
{ \Omega \left( #1 \right) }

\newcommand {\smallOmega} [1]
{ \omega \left( #1 \right) }

\newcommand {\bigTheta} [1]
{ \Theta \left( #1 \right) }

% blank symbol
\newsavebox{\blankbox}
\savebox{\blankbox}{\texttt{aa}}
\newcommand\vartextvisiblespace[1][0.8\wd\blankbox]{%
    \makebox[#1]{\kern.1em\rule{.4pt}{.5ex}%
        \hrulefill%
        \rule{.4pt}{.5ex}\kern.1em}%
}
\newcommand{\blank}{\vartextvisiblespace}% For ease-of-use


\newcommand {\LOGSPACE}
{\mathsf{L}}
\newcommand {\NLOGSPACE}
{\mathsf{NL}}
\newcommand {\PTIME}
{\mathsf{P}}
\newcommand {\NPTIME}
{\mathsf{NP}}
\newcommand {\PSPACE}
{\mathsf{PSPACE}}
\newcommand {\EXPTIME}
{\mathsf{EXP}}
\newcommand {\EXPSPACE}
{\mathsf{EXPSPACE}}

%
% Words
%

\newcommand {\subword}
{\!\preceq}

%
% Automata theory
%

\newcommand {\tow} [1]
{ \xrightarrow{#1} }

\newcommand{\towin}[2]
{\tow{#1}_{#2}}

\DeclareDocumentCommand \lang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL }
    { \calL \left( #1 \right) }
}

\DeclareDocumentCommand \olang { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \calL^\omega }
    { \calL^\omega \!\left( #1 \right) }
}

\DeclareDocumentCommand \Parikh { g } % optinal argument in curly braces
{ 
    \IfNoValueTF {#1}
    { \Psi }
    { \Psi \left( #1 \right) }
}

%
% Grammars
%

% derivation
\newcommand{\derive}{\Rightarrow}
\newcommand{\leftderive}{\derive}

%
% Special
%

\newcommand{\Buechi}{B\"uchi}


==> style/exam.tex <==
% ########################
% EXAM SPECIFIC STUFF
% ########################

% underlining
\usepackage{ulem}
% set emph back to normal (instead of underlined)
\normalem 

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

%
% TOC and hyperlinks
%
\PassOptionsToPackage{obeyspaces}{url}
\usepackage[bookmarksnumbered]{hyperref} 

% border size
\usepackage{geometry}
\geometry{left=2.5cm, right=2.5cm, top=2cm, bottom=2cm, foot= 1cm}

\usepackage[headsepline]{scrlayer-scrpage}
%\clearpairofpagestyles
\clearscrheadfoot
%\ihead{\normalfont \headmark}
\ohead{\hfill \quad \normalfont \page{} \pagemark~/~\Nrpages}
%\automark[]{section}

%
% Dot after section number
%
\usepackage{secdot}
\sectionpunct{subsection}{ }

% space between lines
\onehalfspacing

%
% Hyphenation & separation
%
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%
% Clever references
%

% clever references
\usepackage{cleveref}
% use capital references by default
\let\scref\cref
\let\cref\Cref
% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother
\newcommand{\aemph}[1]{\textit{#1}}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
%\lstset{language=java}
%% Listings
%\lstset{
%    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
%    numbers=left,               % Ort der Zeilennummern
%    numberstyle=\tiny,          % Stil der Zeilennummern
%    %stepnumber=2,               % Abstand zwischen den Zeilennummern
%    numbersep=5pt,              % Abstand der Nummern zum Text
%    tabsize=4,                  % Groesse von Tabs
%    extendedchars=true,         %
%    breaklines=true,            % Zeilen werden Umgebrochen
%    keywordstyle=\text,
%    %frame=b,         
%    stringstyle=\color{black}\ttfamily, % Farbe der String
%    showspaces=false,           % Leerzeichen anzeigen ?
%    showtabs=false,             % Tabs anzeigen ?
%    xleftmargin=5pt,
%    framexleftmargin=17pt,
%    framexrightmargin=5pt,
%    framexbottommargin=4pt,
%    %backgroundcolor=\color{lightgray},
%    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
%    captionpos=t,     
%}
%
%\lstloadlanguages{% Check Dokumentation for further languages ...
%    %[Visual]Basic
%    %Pascal
%    %C
%    %C++
%    %XML
%    %HTML
%    Java
%}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}


%
% Boxes for computational problems
%

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother

\newenvironment{firstpage}
{
    \thispagestyle{empty}
    \newgeometry{top=1cm, bottom=1cm}
}
{
    \pagebreak
    \restoregeometry
}



%
% Exam special stuff
%

\newcommand{\statement}[1]{
    #1	& $\Box$ & $\Box$ \\
}

\newcommand{\maxpts}[1]
{
    \vspace*{-1.5cm}
    \hfill \fbox{\large #1 \pts}
    \vspace*{1cm}
}



% multiplechoice
\newenvironment{multiplechoice}[2]{
    \begin{center}
        \begin{tabular}{lcc}
            & #1 & #2 \\
        }{
        \end{tabular}
    \end{center}
    \vspace{0.5cm}
}

\newenvironment{exerciseDE}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
    
}
{
}

\newenvironment{exerciseEN}[2]
{
    \newpage
    \section{#1}
    \maxpts{#2}
    \vspace*{-0.7cm}
    
}
{
}

\usepackage{verbatim}

\makeatletter
\def\destring{de}
\ifx\style@lang\destring % German

% for comment / endcomment

\newcommand{\exinclude}[1]
{
    \input{exercises/#1}
}

\renewenvironment{exerciseEN}[2]
{
    \comment
}
{
    \endcomment
}


\else % English

\newcommand{\exinclude}[1]
{
    \input{exercises/#1}
}

\renewenvironment{exerciseDE}[2]
{
    \comment
}
{
    \endcomment
}

\fi
\makeatother



==> style/exsheet.tex <==
% ##############################
% EXERCISE SHEET SPECIFIC STUFF
% ##############################

%
% Bibliography & references
%

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,maxbibnames=9,maxcitenames=9,backend=bibtex,giveninits=true,isbn=false,doi=false]{biblatex}
\DeclareFieldFormat*{title}{\mkbibitalic{#1\isdot}}
\DeclareFieldFormat*{booktitle}{#1\isdot}
\DeclareFieldFormat*{journaltitle}{#1\isdot}
%\DeclareFieldFormat{titlecase}{\MakeSentenceCase{#1}}
%\newbibmacro*{journal}{%
%    \iffieldundef{journaltitle}
%    {}
%    {\printtext[journaltitle]{%
%            \printfield[noformat]{journaltitle}%
%            \setunit{\subtitlepunct}%
%            \printfield[noformat]{journalsubtitle}}}}

%
% Includes
%

% underlining
\usepackage{ulem}
% set emph back to normal (instead of underlined)
\normalem 

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% border size
\usepackage[]{geometry}
\geometry{left=2.2cm, right=2.2cm, top=2cm, bottom=2cm, foot= 1cm}

%
% emph as bold
%

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother
\newcommand{\aemph}[1]{\textit{#1}}

%
% Clever references
%

% clever references
\usepackage{cleveref}
% use capital references by default
\let\scref\cref
\let\cref\Cref

\usepackage{scrlayer-scrpage}
\clearscrheadfoot

% space between lines
\onehalfspacing

%
% Hyphenation & separation
%
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%
% Redefined environment
%

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
    {paragraph} % name
    {4}         % level
    {\z@}       % indent     
    {0ex \@plus -1ex \@minus -.2ex} % beforeskip
    %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
    {0.01ex \@plus .2ex}                % afterskip
    %{1.5ex \@plus -2ex}                % afterskip
    {\normalfont\normalsize\bfseries} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% shortproof without newline
\makeatletter
\newenvironment{shortproof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother


%
% Theorem styles
%

% Theoremstyle
\newtheoremstyle{withnumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1 #2\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\newtheoremstyle{nonumber} % name
{0.4cm}                    % Space above
{0.6cm}                    % Space below
{\normalfont}                   % Body font
{}                           % Indent amount
{\bfseries}                   % Theorem head font
{\newline}                          % Punctuation after theorem head
{0.2cm}                       % Space after theorem head
{#1\thmnote{: \ #3}}  % Theorem head spec (can be left empty, meaning ‘normal’)

\theoremstyle{withnumber} 

%
% Hackfix for itemize / enumerate at the beginning of a theorem
%
\newcommand{\skipfix}{\leavevmode\vspace{-2.2em}}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \skipfix
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \skipfix
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
%\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }

% captions
%\usepackage{capt-of}
%\usepackage{caption}
%\DeclareCaptionFont{white}{\color{white}}
%\DeclareCaptionFormat{listing}
%{
%    \colorbox[cmyk]{1, 1, 1,0.01}
%    {
%        \parbox{\textwidth}
%        {\hspace{15pt}#1#2#3}
%    }
%}
%\captionsetup[lstlisting]
%{
%    format=listing,
%    labelfont=white,
%    textfont=white,
%    singlelinecheck=false,
%    margin=0pt,
%    font={bf,footnotesize}
%}

% listings
%\usepackage{listings}
%\lstset{
%    numbers=left,
%    numberstyle=\tiny,
%    numbersep=5pt,
%    keywordstyle=\color{black}\bfseries,
%    stringstyle=\ttfamily,
%    showstringspaces=false,
%    basicstyle=\footnotesize,
%    captionpos=b
%}
%\lstset{language=java}
%% Listings
%\lstset{
%    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
%    numbers=left,               % Ort der Zeilennummern
%    numberstyle=\tiny,          % Stil der Zeilennummern
%    %stepnumber=2,               % Abstand zwischen den Zeilennummern
%    numbersep=5pt,              % Abstand der Nummern zum Text
%    tabsize=4,                  % Groesse von Tabs
%    extendedchars=true,         %
%    breaklines=true,            % Zeilen werden Umgebrochen
%    keywordstyle=\text,
%    %frame=b,         
%    stringstyle=\color{black}\ttfamily, % Farbe der String
%    showspaces=false,           % Leerzeichen anzeigen ?
%    showtabs=false,             % Tabs anzeigen ?
%    xleftmargin=5pt,
%    framexleftmargin=17pt,
%    framexrightmargin=5pt,
%    framexbottommargin=4pt,
%    %backgroundcolor=\color{lightgray},
%    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
%    captionpos=t,     
%}
%\lstloadlanguages{% Check Dokumentation for further languages ...
%    %[Visual]Basic
%    %Pascal
%    %C
%    %C++
%    %XML
%    %HTML
%    Java
%}

%
% Colors
%

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}

%
% Boxes for computational problems
%

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}

\makeatother
\newtoks\lecturer
\newtoks\organizer
\newtoks\institution
\newtoks\term
\newtoks\releasedate
\newtoks\duedate

\makeatletter
\newcommand{\head}
{
    %   \newgeometry{top=1cm}
    \vspace*{-3\baselineskip}
    %\null
    %\thispagestyle{empty}
    %\begin{center} 
    \framebox[\textwidth]{
        \parbox{\textwidth}
        {
            \vspace*{-0.2cm}
            \begin{center}
                \textrm{\textbf{\large \@title}} \\
                \textrm{\textbf{\large \@subtitle}}
            \end{center}
            \vspace*{-0.9cm}
            \begin{tabu} to \textwidth {l X r}
                \small \the\lecturer  & & \small \the\institution \\
                \small \the\organizer  & & \small \the\term \\
            \end{tabu}
        }
    } 
    %\end{center}
    %\null
    \begin{tabu} to \textwidth {@{} l X r @{}}
        \the\releasedate  & & \the \duedate \\
    \end{tabu}
    %    \vspace*{0.2cm}
    %    \restoregeometry
}
\makeatother


==> style/helvetica.tex <==
% #######
% HELVETICA
% #######

% Helvetica pro for text (and math)
% Consolas for monospace
% Euler for math

\usepackage{helvet}
\renewcommand{\familydefault}{\sfdefault}

\usepackage{isomath}
\usepackage{sansmathfonts}


==> style/ieee_additions.tex <==
% #####################
% ADDITIONS FOR IEEE
% #####################

% enumerate[a)] etc
\usepackage{paralist}

% define theorem styles
\theoremstyle{plain}

\newtheorem {theorem}       {Theorem}     []
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Exercise}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

% separation rules
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

%compact llncs-like paragraph
\newcommand{\compactparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}

\newcommand{\subparagraph}[1]{%
    \medskip%
    \noindent%
    {\bf \sffamily #1.}%
}


==> style/includes.tex <==
% ##########
% INCLUDES
% ##########

% images, ...
\usepackage{graphicx}

% tables (over several pages)
\usepackage{tabu}

% boxes in the text
\usepackage{fancybox}

% math symbols
\usepackage{amsmath}
%\usepackage{amssymb}
\usepackage{stmaryrd} 
\usepackage{amsthm}
\usepackage{wasysym}
\usepackage{marvosym}

% for coloring stuff
\usepackage{xcolor}

% for colored cells in tables
\usepackage{colortbl}

% symbol scaling in math mode
\usepackage{scalerel}

% for symbol stacking
\usepackage{stackengine}

% parse optional arguments
\usepackage{xparse}

% fix some spacing issues
\usepackage{microtype}

% custom environments
\usepackage{environ}


==> style/lang_de.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: DEUTSCH
% ###################################

%
% Packages
%

%\usepackage{polyglossia}
%\setdefaultlanguage{german}

%\usepackage[ngerman]{babel}

\usepackage[utf8]{inputenc}
\usepackage{csquotes}

%
% Quotes
%

\newcommand {\quot} [1] {\enquote{#1}}

%
% Commands
%

\newcommand{\pts}{Punkte}
\newcommand{\page}{Seite}
\newcommand{\ProblemLocGiven}{Gegeben}
\newcommand{\ProblemLocDecide}{Entscheide}
\newcommand{\ProblemLocCompute}{Berechne}




==> style/lang_en.tex <==
% ###################################
% LANGUAGE DEPENDANT STUFF: ENGLISH
% ###################################

%
% Packages
%

\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage{csquotes}


%
% Quotes
% 

\newcommand {\quot} [1] {\enquote{#1}}

%
% Commands
%

\newcommand{\pts}{points}
\newcommand{\page}{Page}
\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}



==> style/letter.tex <==
% ########################
% ARTICLE SPECIFIC STUFF
% ########################

% Festlegung Art der Zitierung - Havardmethode: Abkuerzung Autor + Jahr
\usepackage[style=alphabetic,backend=bibtex]{biblatex}

% underlining
\usepackage{ulem}

% remove all paragraph indentation
\usepackage{parskip}

% spacing between lines of text
\usepackage{setspace}

% enumerate etc
\usepackage{paralist}

% keyword index
\usepackage{makeidx}

% create keyword index
\makeindex

% abbreviation index
\usepackage[german]{nomencl}
\let\abbrev\nomenclature

% border size
\usepackage{geometry}
% top is later changed, just for title page
\geometry{left=2.5cm, right=2.5cm, top=2.5cm, bottom=2cm, foot= 1cm}

% Indentation
% space between lines
\onehalfspacing
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000

%\usepackage{scrpage2}
%\pagestyle{scrheadings}
%\cfoot{\pagemark}

%  headline / footline
\usepackage{fancyhdr} %Paket laden
\pagestyle{fancy} %eigener Seitenstil

%% Seitennummer immer oben rechts
%% alle Kopf- und Fußzeilenfelder bereinigen
%\fancyhf{}
%% Kopfzeile links: Name des Kapitels = der Sektion
%\fancyhead[L]{\nouppercase{\leftmark}}
%% Kopfzeile zentriert:
%\fancyhead[C]{} 
%% Kopfzeile rechts = Seitennummer
%\fancyhead[R]{\thepage} 
%% Trennlinien
%\renewcommand{\headrulewidth}{0.4pt} 
%%\renewcommand{\footrulewidth}{0.4pt}
%% Analog
%%\fancyfoot[C]{\thepage}


% Seitennummer immer oben rechts
% alle Kopf- und Fußzeilenfelder bereinigen
\fancyhf{}
\fancyfoot[C]{\thepage}
\renewcommand{\headrule}{} 

% references
\usepackage[bookmarksnumbered]{hyperref} 

% line break in URLs
%\usepackage[hyphens,obeyspaces,spaces]{url}

% newline after paragraph, paragraph bold and underlined
\makeatletter
\renewcommand {\paragraph}
{
    \@startsection
        {paragraph} % name
        {4}         % level
        {\z@}       % indent     
        {0ex \@plus -1ex \@minus -.2ex} % beforeskip
        %{-3.25ex\@plus -1ex \@minus -.2ex} % beforeskip
        {0.01ex \@plus .2ex}                % afterskip
        %{1.5ex \@plus -2ex}                % afterskip
        {\normalfont\normalsize\bfseries\underbar} % style of heading
}
\makeatother

% proof in bold font, colon and newline afterwards
\makeatletter
\renewenvironment{proof}[1][\proofname]
{
    \par
    \pushQED{\qed}%
    \normalfont \topsep6\p@\@plus6\p@\relax
    \trivlist
    \item[\hskip\labelsep\bfseries
    #1:]\mbox{}\\*\ignorespaces% ADDED
}
{
    \popQED\endtrivlist\@endpefalse
}
\makeatother

% set emph back to normal (instead of underlined)
\normalem 

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

% Theorem numbering
\def\theoremnumberstyle{changesection}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Zu verwendende Regelsaetze 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Bei Nummerierung vom Typ swapped soll abweichend vom Standard
%%% "5.12. Satz" erscheinen als "5.12 Satz", das heisst ohne
%%% zusaetzlichen Punkt.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\def\swappedhead#1#2#3{%
%    \thmnumber{#2}\thmname{\@ifnotempty{#2}{ }#1}%
%    \thmnote{ {\the\thm@notefont(#3)}}}

\def\swappedhead#1#2#3{%
    \thmnumber{#2}\thmname{ #1}%
    \thmnote{ {\the\thm@notefont(#3)}}}

\newtheoremstyle{varthm-roman-break}% name
{}%      Space above, empty = `usual value'
{}%      Space below
{\normalfont}% Body font
{}%         Indent amount (empty = no indent, \parindent = para indent)
{\bfseries}% Thm head font
{}%        Punctuation after thm head
{\newline}%     Space after thm head: " " = normal interword space;
%       \newline = linebreak
{\thmnote{#3}}% Thm head spec


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% Eigene Befehle
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Label an beliebiger Stelle mit beliebigem Symbol setzen
% \mylabel{labelname}{(*)} liefert (*) nach \ref{labelname}
\catcode`@=11%%% Sorgt daruer, dass @ in Marconamen verwendet werden kann
\newcommand{\mylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}}}%
    \@esphack}
\newcommand{\tmylabel}[2]{\@bsphack
    \protected@write\@auxout{}%
    {\string\newlabel{#1}{{#2}{\thepage}{\arabic{chapter}}}}%
    \@esphack}
\catcode`@=\active%
%%% Erzeugt an der Stelle des Aufrufs einen nicht sichtbaren Punkt.
\newcommand{\leererpunkt}{
    \drawdim pt
    \begin{texdraw}
        \setgray 1
        \lcir r:0.01       
    \end{texdraw}
}

\swapnumbers
\theoremstyle{varthm-roman-break} 

\newtheorem {theorem}	    {Theorem}     [section]
\newtheorem {corollary}		[theorem]     {Corollary}
\newtheorem {lemma}			[theorem]     {Lemma}
\newtheorem {proposition}	[theorem]     {Proposition}
\newtheorem {remark}		[theorem]     {Remark}
\newtheorem {definition}	[theorem]     {Definition}
\newtheorem {notation}		[theorem]     {Notation}
\newtheorem {example}		[theorem]     {Example}
\newtheorem {exercise}		[theorem]     {Example}
\newtheorem {algo}			[theorem]     {Algorithm}
\newtheorem {claim}			[theorem]     {Claim}

% itemize/enumerate at the beginning of a thm
\newenvironment{thmenumerate}
{
    \leavevmode\vspace{-1.4em}
    \begin{enumerate}
    }
    {
    \end{enumerate}
}

\newenvironment{thmitemize}
{
    \leavevmode\vspace{-1.4em}
    \begin{itemize}
    }
    {
    \end{itemize}
}

% chapters = sections (otherwise numbering will not work)
\let\chapter\section

% subsections numbered by capital arabic letters
%\renewcommand{\thesubsection}{\thesection.\Roman{subsection}}
\renewcommand{\thesubsection}{\Alph{subsection})}

\usepackage{secdot}
\sectionpunct{subsection}{ }


% captions
\usepackage{capt-of}
\usepackage{caption}
\DeclareCaptionFont{white}{\color{white}}
\DeclareCaptionFormat{listing}
{
    \colorbox[cmyk]{1, 1, 1,0.01}
    {
        \parbox{\textwidth}
        {\hspace{15pt}#1#2#3}
    }
}
\captionsetup[lstlisting]
{
    format=listing,
    labelfont=white,
    textfont=white,
    singlelinecheck=false,
    margin=0pt,
    font={bf,footnotesize}
}

% listings
\usepackage{listings}
\lstset{
    numbers=left,
    numberstyle=\tiny,
    numbersep=5pt,
    keywordstyle=\color{black}\bfseries,
    stringstyle=\ttfamily,
    showstringspaces=false,
    basicstyle=\footnotesize,
    captionpos=b
}
\lstset{language=java}
% Listings
\lstset{
    basicstyle=\fontsize{9}{9}\ttfamily, % Standardschrift
    numbers=left,               % Ort der Zeilennummern
    numberstyle=\tiny,          % Stil der Zeilennummern
    %stepnumber=2,               % Abstand zwischen den Zeilennummern
    numbersep=5pt,              % Abstand der Nummern zum Text
    tabsize=4,                  % Groesse von Tabs
    extendedchars=true,         %
    breaklines=true,            % Zeilen werden Umgebrochen
    keywordstyle=\text,
    %frame=b,         
    stringstyle=\color{black}\ttfamily, % Farbe der String
    showspaces=false,           % Leerzeichen anzeigen ?
    showtabs=false,             % Tabs anzeigen ?
    xleftmargin=5pt,
    framexleftmargin=17pt,
    framexrightmargin=5pt,
    framexbottommargin=4pt,
    %backgroundcolor=\color{lightgray},
    showstringspaces=false,      % Leerzeichen in Strings anzeigen ?
    captionpos=t,     
}

\lstloadlanguages{% Check Dokumentation for further languages ...
    %[Visual]Basic
    %Pascal
    %C
    %C++
    %XML
    %HTML
    Java
}

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}


\newtoks\receiver
\newtoks\address
\newtoks\postalbox
\newtoks\plz
\newtoks\telnr
\newtoks\email

\catcode`\@ = 11 % Macro \makeatletter does the same

%\newcommand{ \at } { \makeatletter @ \makeatother }

\newcommand {\letterhead}
{
    
    \begin{tabu} to \textwidth {lXr}
        \large \the\receiver       & & \large Sebastian Muskalla\\
        \small \the\address     & & \small Institut für Theoretische Informatik\\
        \small \the\postalbox  & & \small Mühlenpfordtstr. 23\\
        \small \the\plz       & & \small 38106 Braunschweig\\
        \small \the\telnr     & & \small Tel.:  +49 (0)531 391 9520 \\
        \small \the\email     & & \small E-Mail: s.muskalla{\!\at \!}tu-bs.de\\
                                & & \\
                                & & Braunschweig, den \today \\
    \end{tabu}
    \makeatother
}

\newcommand {\lettertitle}
{\mbox{}\\\textbf{\Large{\@title}}\\}




==> style/lipics_additions.tex <==
% #####################
% ADDITIONS FOR LIPICS
% #####################
% some paper specific stuff

% enumerate[a)] etc.
\usepackage{paralist}

\theoremstyle{plain}
\newtheorem {proposition} [theorem] {Proposition}
\newtheorem {claim} [theorem] {Claim}

\theoremstyle{definition}
\newtheorem {algo} [theorem] {Algorithm}
\newtheorem {rmk} [theorem] {Remark}

% separation rules
\sloppy % Never violate page margin
\clubpenalty = 10000 % Disable single lines at the start of a paragraph (Schusterjungen)
\widowpenalty = 10000 % Disable single lines at the end of a paragraph (Hurenkinder)
\displaywidowpenalty = 10000
\binoppenalty = 10000 % Disable separating math operators 
\relpenalty = 10000 % Disable separating math relations

% Quotes
\newcommand {\quot} [1] {\enquote{#1}}


% Boxes for computation problems
%
%
\newcommand{\ProblemLocGiven}{Given}
\newcommand{\ProblemLocDecide}{Decide}
\newcommand{\ProblemLocCompute}{Compute}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question


\NewEnviron{problem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \sffamily
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \sffamily
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/misc.tex <==
% ##########
% MISC
% ##########

%
% Fix delimiter spacing
%
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}

%
% Custom symbols
%

% triangle qed
\newcommand{\tqed}{\hfill \text{$\blacktriangleleft$}}

% item with arrow symbol like in Meyer's lectures
\newcommand {\itemarrow} 
{ {\raisebox{0.8mm}{\rotatebox[origin=c]{180}{$\Lsh$}}} } 

%
% Use slanted versions of leq & geq by default
%

% store old symbols
\let\leqstraight\leq % or just use le
\let\geqstraight\geq % or just use ge
\let\nleqstraight\nleq
\let\ngeqstraight\ngeq
\let\nle\nleq
\let\nge\ngeq

% overwrite
\let\leq\leqslant
\let\geq\geqslant
\let\nleq\leqslant
\let\ngeq\ngeqslant


==> style/myriad.tex <==
% #######
% MYRIAD
% #######

%
% Use Myriad Pro for text and math
%

% MdSymbol for math symbols that work well together with Myriad Pro
\usepackage{mdsymbol}

% Mathspec to change fonts for math and text
% (loads fontspecc with no-math option)
\usepackage{mathspec}

% Use Myriad Pro for text
\setmainfont{Myriad Pro}
\setsansfont{Myriad Pro}

% Use Myriad Pro for math
\setmathsfont(Digits,Latin,Greek){Myriad Pro}
\setmathrm{Myriad Pro}
\setmathsf{Myriad Pro}

% Use Consolas as monospace / typewriter font for text an math
\setmonofont{Consolas}
\setmathtt{Consolas}

% the greek symbols provided by Myriad Pro already look like their standard-LaTeX var-variants
\let\oldvarepsilon\varepsilon
\let\oldvarphi\varphi
\let\varepsilon\epsilon
\let\varphi\phi

% Load font styles for math that are not included in Myriad Pro
% Blackboard bold: Boondox (which is based on STIX)
% Calligraphic: Computer Modern (simply the best...)
% Fraktur: Boondox (which is based on STIX)
% Boondox (based on stix) for, fraktur and script
% Script: Boondox
\usepackage
[
    cal=cm,
    bb=boondox,
    frak=boondox,
    scr=boondoxo
]
{mathalfa}

\let\oldell\ell
\renewcommand{\ell}{\mathscr{l}}

% bm for bold math
% does not work with greek letters - but Myriad Pro provides bold greek letters, available using \mathbf
\usepackage{bm}

% hack for correct bold Greek letters

\newcommand{\bAlpha}{\bm{Alpha}}

%$\Alpha \Beta \Gamma \Delta \Epsilon \Zeta \Eta \Theta \Iota \Kappa \Lambda \Mu \Nu \Xi O \Pi \Rho \Sigma \Tau \Upsilon \Phi \Chi \Psi \Omega$\\
%$\alpha \beta \gamma \delta \epsilon \zeta \eta \theta \iota \kappa \lambda \mu \nu \xi o \pi \rho \sigma \tau \upsilon \phi \chi \psi \omega$



%
% Old hacks
%

% hack for emptyset
% (not needed for mdsymbol)
%\renewcommand{\emptyset}{ {\diameter} }

% make calligraphic bold
%\let\mathcal\mathbcal


==> style/nth.tex <==
% nth.sty  version 2002/27/02 Donald Arseneau
% Ordinal numbering style, 1st 2nd 3rd 4th 5th... 12th... 101st 102nd...
%
% (Public domain: take, include, extract, whatever)
%
% In LaTeX: 
%           \usepackage[super,negative]{nth}
% where option [super] gives superscript `th'
% and option [negative] allows ``st, nd, rd'' suffixes on negative numbers.
%
% example:  \renewcommand{\thesection}{\ordinal{section}}
% or        \renewcommand{\thesection}{\@ordinal\c@section}
% or        \renewcommand{\thesection}{\nth\c@section}
%   
% In plain TeX: 
%           \input nth.sty
% use:      \nth{<number>}.
% Change formatting by redefining \nthscript and \nthtest

% modified to be also able to do things like \nth{i}
% (in this case, always "th" is used)

% ToDo:
% \nth{(n+1)} should give (n+1)^st

\usepackage{xstring}

% optionally specify desired subscript
\DeclareDocumentCommand \nth { m g } % optinal argument in curly braces
{%
    \IfNoValueTF {#2}%
    {%
        \IfInteger{#1}%
        {\nthH{#1}}%
        {{#1\nthscript{th}}}%
    }%
    {%
        {#1\nthscript{#2}}%
    }%
}%


\def\nthH#1{% First print number:
    \expandafter\nthM \number #1\relax
    \nthscript{%
        \ifnum#1\nthtest0 th\else % negatives are all ``th'' (depending on \nthtest)
        \expandafter \nthSuff \expandafter 0\number\ifnum #1<0-\fi#1\delimiter
        \fi
    }}
    
% Minus sign using math mode:
\def\nthM#1{\if -#1\ifmmode-\else$-$\fi\else #1\fi}

% Print suffix depending on last two digits:
\def\nthSuff#1#2#3{%
    \ifx \delimiter#3% #1#2 are last two digits
    \ifnum #1=1 th%  teens are always ``th''
    \else % use appropriate suffix
    \ifcase #2 th\or st\or nd\or rd\else th\fi
    \fi
    \else % continue scanning for last two digits
    \expandafter \nthSuff \expandafter #2\expandafter #3%
    \fi}

% Formatting hook for ordinals (\let\nthscript\textsuperscript)
\def\nthscript#1{\textsuperscript{#1}}% alternate: \def\nthscript#1{$\rm^{#1}$}

% Formatting hook for all negative numbers giving ``th''
\def\nthtest{=}  % alternate: \def\nthtest{>}


==> style/operators.tex <==
% ##################
% OPERATORS
% ##################

%\DeclareMathOperator{\Attr}{Attr}
\DeclareMathOperator{\bin}{bin}


==> style/presentation.tex <==
% #######################
% BEAMER SPECIFIC STUFF
% #######################

% Metropolis theme
% (has to be installed)
\usetheme{metropolis}

% ???
\usepackage{booktabs}
\usepackage[scale=2]{ccicons}

% stuff for tikz
\usepackage{pgfplots}
\usepgfplotslibrary{dateplot}

% absolute positioning of boxes
\usepackage[absolute,overlay]{textpos}

% enumeration
\usepackage{enumerate}

% emph as bold
\makeatletter
\DeclareRobustCommand{\em}{%
    \@nomath\em \if b\expandafter\@car\f@series\@nil
    \normalfont \else \bfseries \fi}
\makeatother

\definecolor{myblue}{HTML}{3399FF}
\definecolor{mybluefaded}{HTML}{99CCFF}
\definecolor{myred}{HTML}{FF3333}
\definecolor{myredfaded}{HTML}{FF9999}
\definecolor{myblue}{HTML}{3399FF}
\definecolor{tubsred}{HTML}{BE1E06}
\definecolor{feuervogel}{HTML}{B24f4D}

\makeatletter
\newcommand {\problemtitle}[1]{\gdef\@problemtitle{#1}}% Store problem title
\newcommand {\problemshort}[1]{\gdef\@problemshort{#1}}% Store problem short notation
\newcommand {\probleminput}[1]{\gdef\@probleminput{#1}}% Store problem input
\newcommand {\problemparameter}[1]{\gdef\@problemparameter{#1}}% Store problem parameter
\newcommand {\problemquestion}[1]{\gdef\@problemquestion{#1}}% Store problem question

\NewEnviron{decproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocDecide:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\NewEnviron{compproblem}{%
    \problemtitle{}\problemshort{}\probleminput{}\problemquestion{}% Default input is empty
    \BODY% Parse input
    \par\addvspace{.5\baselineskip}
    \noindent
    %    
    \framebox[1\columnwidth]{%15.00002pt is the former size of parindent
        \hspace*{2em}
        \begin{tabu} to 1\columnwidth {@{\hspace{\parindent}} l X c}
            \multicolumn{2}{@{\hspace{\parindent}}l}{ \normalsize \textbf{\underline{\@problemtitle}} \@problemshort} \\% Title and shortcut
            \normalsize \textbf{\ProblemLocGiven:} & \normalsize \@probleminput \\% Input
            \normalsize \textbf{\ProblemLocCompute:} & \normalsize \@problemquestion% Question
        \end{tabu}
    }
    
    \par\addvspace{.5\baselineskip}
}
\makeatother


==> style/stix.tex <==
% #######
% STIX
% #######


% - myriad for text and math
% - consolas for monospace
% - euler for greek letters

% REQUIRES XELATEX!

% Consolas and Myriad Pro have to be installed

% Myriad pro for text (and math)
% Consolas for monospace
% Euler for math

\usepackage[notext]{stix}

% package to change font in XeTeX
\usepackage[no-math]{fontspec}

% euler font for math
%\usepackage[mathbf]{euler}
    
% default font: Myriad pro
% (has to be installed!)
\setmainfont{Myriad Pro}
\setsansfont{Myriad Pro}
\newfontfamily\myriad{Myriad Pro}

% monospace font: Consolas
% (has to be installed!)
\setmonofont{Consolas}

% use normal text font for math
%\usepackage[noendash,italic]{mathastext}

% hack for emptyset
\renewcommand{\emptyset}{ {\diameter} }

% font for section, part, ... titles (in text and in table of contents)
\usepackage{titlesec}
\addtokomafont{title}{\myriad}
\setkomafont{subsection}{\bfseries\Large\myriad}
\setkomafont{section}{\bfseries\huge\myriad}
\setkomafont{sectionentry}{\bfseries\myriad} % entry in TOC
\setkomafont{part}{\bfseries\Huge\myriad} % part name
\setkomafont{partnumber}{\bfseries\Huge\myriad} % "Part II."
\setkomafont{partentry}{\bfseries\large\myriad} % entry in TOC
\setkomafont{paragraph}{\bfseries\myriad}
\setkomafont{subparagraph}{\bfseries\myriad} % entry in TOC

% Take nice sans-serif greek letters from the font "Euler"
%\DeclareSymbolFont{EulerGreek}{U}{eur}{m}{n}
%\DeclareMathSymbol\Gamma    {\mathalpha}{EulerGreek}{"00}
%\DeclareMathSymbol\Delta    {\mathalpha}{EulerGreek}{"01}
%\DeclareMathSymbol\Theta    {\mathalpha}{EulerGreek}{"02}
%\DeclareMathSymbol\Lambda   {\mathalpha}{EulerGreek}{"03}
%\DeclareMathSymbol\Xi       {\mathalpha}{EulerGreek}{"04}
%\DeclareMathSymbol\Pi       {\mathalpha}{EulerGreek}{"05}
%\DeclareMathSymbol\Sigma    {\mathalpha}{EulerGreek}{"06}
%\DeclareMathSymbol\Upsilon  {\mathalpha}{EulerGreek}{"07}
%\DeclareMathSymbol\Phi      {\mathalpha}{EulerGreek}{"08}
%\DeclareMathSymbol\Psi      {\mathalpha}{EulerGreek}{"09}
%\DeclareMathSymbol\Omega    {\mathalpha}{EulerGreek}{"0A}
%\DeclareMathSymbol{\alpha}  {\mathalpha}{EulerGreek}{"0B}
%\DeclareMathSymbol{\beta}   {\mathalpha}{EulerGreek}{"0C}
%\DeclareMathSymbol{\gamma}  {\mathalpha}{EulerGreek}{"0D}
%\DeclareMathSymbol{\delta}  {\mathalpha}{EulerGreek}{"0E}
%\DeclareMathSymbol{\epsilon}{\mathalpha}{EulerGreek}{"0F}
%\DeclareMathSymbol{\zeta}   {\mathalpha}{EulerGreek}{"10}
%\DeclareMathSymbol{\eta}    {\mathalpha}{EulerGreek}{"11}
%\DeclareMathSymbol{\theta}  {\mathalpha}{EulerGreek}{"12}
%\DeclareMathSymbol{\iota}   {\mathalpha}{EulerGreek}{"13}
%\DeclareMathSymbol{\kappa}  {\mathalpha}{EulerGreek}{"14}
%\DeclareMathSymbol{\lambda} {\mathalpha}{EulerGreek}{"15}
%\DeclareMathSymbol{\mu}     {\mathalpha}{EulerGreek}{"16}
%\DeclareMathSymbol{\nu}     {\mathalpha}{EulerGreek}{"17}
%\DeclareMathSymbol{\xi}     {\mathalpha}{EulerGreek}{"18}
%\DeclareMathSymbol{\pi}     {\mathalpha}{EulerGreek}{"19}
%\DeclareMathSymbol{\rho}    {\mathalpha}{EulerGreek}{"1A}
%\DeclareMathSymbol{\sigma}  {\mathalpha}{EulerGreek}{"1B}
%\DeclareMathSymbol{\tau}    {\mathalpha}{EulerGreek}{"1C}
%\DeclareMathSymbol{\upsilon}{\mathalpha}{EulerGreek}{"1D}
%\DeclareMathSymbol{\phi}    {\mathalpha}{EulerGreek}{"1E}
%\DeclareMathSymbol{\chi}    {\mathalpha}{EulerGreek}{"1F}
%\DeclareMathSymbol{\psi}    {\mathalpha}{EulerGreek}{"20}
%\DeclareMathSymbol{\omega}  {\mathalpha}{EulerGreek}{"21}
%\DeclareMathSymbol{\varepsilon}{\mathalpha}{EulerGreek}{"22}
%\DeclareMathSymbol{\vartheta}{\mathalpha}{EulerGreek}{"23}
%\DeclareMathSymbol{\varpi}  {\mathalpha}{EulerGreek}{"24}
%\DeclareMathSymbol{\varphi} {\mathalpha}{EulerGreek}{"27}
%\DeclareMathSymbol\upOmega  {\mathord}{EulerGreek}{"0A}
%\DeclareMathSymbol\upDelta  {\mathord}{EulerGreek}{"01}

% blackbord bold letters
%\DeclareMathAlphabet{\mathds}{U}{dsrom}{m}{n}
\usepackage[bb=fourier]{mathalfa}


==> style/theorems_de.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}      [theorem]     {Theorem}
\newtheorem {corollary}     [theorem]     {Korollar}
\newtheorem {lemma}         [theorem]     {Lemma}
\newtheorem {proposition}   [theorem]     {Proposition}
\newtheorem {remark}        [theorem]     {Bemerkung}
\newtheorem {definition}    [theorem]     {Definition}
\newtheorem {notation}      [theorem]     {Notation}
\newtheorem {example}       [theorem]     {Beispiel}
\newtheorem {exercise}      [theorem]     {Aufgabe}
\newtheorem {algo}          [theorem]     {Algorithm}
\newtheorem {claim}         [theorem]     {Behauptung}
\newtheorem {conjecture}    [theorem]     {Hypothese}
\newtheorem {sources}       [theorem]     {Quellen}
\newtheorem {defprop}       [theorem]     {Definition \& Proposition}
\newtheorem {deflemma}      [theorem]     {Definition \& Lemma}
\newtheorem {deftheorem}    [theorem]     {Definition \& Theorem}

\theoremstyle{nonumber} 

\newtheorem* {theorem*}         {Theorem}
\newtheorem* {corollary*}       {Korollar}
\newtheorem* {lemma*}           {Lemma}
\newtheorem* {proposition*}     {Proposition}
\newtheorem* {remark*}          {Bemerkung}
\newtheorem* {definition*}      {Definition}
\newtheorem* {notation*}        {Notation}
\newtheorem* {example*}         {Beispiel}
\newtheorem* {exercise*}        {Aufgabe}
\newtheorem* {algo*}            {Algorithm}
\newtheorem* {claim*}           {Behauptung}
\newtheorem* {conjecture*}      {Hypothese}
\newtheorem* {sources*}	        {Quellen}
\newtheorem* {defprop*}         {Definition \& Proposition}
\newtheorem* {deflemma*}        {Definition \& Lemma}
\newtheorem* {deftheorem*}      {Definition \& Theorem}

\theoremstyle{withnumber} 


==> style/theorems_en.tex <==
% ######################
% THEOREM ENVIRONMENTS
% ######################

%\newtheorem {theorem}      [theorem]     {Theorem}
\newtheorem {corollary}     [theorem]     {Corollary}
\newtheorem {lemma}         [theorem]     {Lemma}
\newtheorem {proposition}   [theorem]     {Proposition}
\newtheorem {remark}        [theorem]     {Remark}
\newtheorem {definition}    [theorem]     {Definition}
\newtheorem {notation}      [theorem]     {Notation}
\newtheorem {example}       [theorem]     {Example}
\newtheorem {exercise}      [theorem]     {Exercise}
\newtheorem {algo}          [theorem]     {Algorithm}
\newtheorem {claim}         [theorem]     {Claim}
\newtheorem {conjecture}    [theorem]     {Conjecture}
\newtheorem {sources}       [theorem]     {Sources}
\newtheorem {defprop}       [theorem]     {Definition \& Proposition}
\newtheorem {deflemma}      [theorem]     {Definition \& Lemma}
\newtheorem {deftheorem}    [theorem]     {Definition \& Theorem}

\theoremstyle{nonumber} 

\newtheorem* {theorem*}         {Theorem}
\newtheorem* {corollary*}       {Corollary}
\newtheorem* {lemma*}           {Lemma}
\newtheorem* {proposition*}     {Proposition}
\newtheorem* {remark*}          {Remark}
\newtheorem* {definition*}      {Definition}
\newtheorem* {notation*}        {Notation}
\newtheorem* {example*}         {Example}
\newtheorem* {exercise*}        {Exercise}
\newtheorem* {algo*}            {Algorithm}
\newtheorem* {claim*}           {Claim}
\newtheorem* {conjecture*}      {Conjecture}
\newtheorem* {sources*}	        {Sources}
\newtheorem* {defprop*}         {Definition \& Proposition}
\newtheorem* {deflemma*}        {Definition \& Lemma}
\newtheorem* {deftheorem*}      {Definition \& Theorem}

\theoremstyle{withnumber} 


==> style/tikz.tex <==
% ########################
% TIKZ
% ########################

% Includes
\usepackage{tikz}
\usepackage{pgf}
\usepackage{tikz-dependency}
\usetikzlibrary{arrows}
\usetikzlibrary{automata}
\usetikzlibrary{shapes}
\usetikzlibrary{backgrounds}
\usetikzlibrary{petri}
\usetikzlibrary{calc} 
\usetikzlibrary{decorations}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.pathreplacing}
\usetikzlibrary{positioning}
\usetikzlibrary{patterns}
\usetikzlibrary{petri}
\usetikzlibrary{fit}
\usetikzlibrary{graphs} 
\usetikzlibrary{calc}
\usetikzlibrary{tikzmark}

\tikzset{
    treenode/.style = {align=center, inner sep=0pt, text centered,
        font=\sffamily},
    roundpos/.style = {treenode, circle, black, draw=black,
        minimum size=2.5em},
    squarepos/.style = {treenode, rectangle, black, draw=black,
        minimum width=2em, minimum height=2em},
}

\tikzset{
    invisible/.style={opacity=0},
    visible on/.style={alt={#1{}{invisible}}},
    alt/.code args={<#1>#2#3}{%
        \alt<#1>{\pgfkeysalso{#2}}{\pgfkeysalso{#3}} % \pgfkeysalso doesn't change the path
    },
}

%
% Transition Boxes
%
\tikzset
{
    tboxoutline/.style = 
    {
        draw,
        thick,
        minimum size=6em,
        inner sep=0pt,
        outer sep=0pt,
    },
    tboxstate/.style =
    {
        minimum width=4pt,
        minimum height=2pt,
        inner sep=0pt,
        fill
    },
    tboxarrow/.style =
    {
    },
    pics/tbox/.style 2 args =
    {
        code =
        {
            \node[tboxoutline,pic actions] (-box) {};
            \foreach \i in {1,...,#1}
            {
                \path
                    (-box.north west)
                    --
                    node
                        [tboxstate,anchor=east,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-in-\i)
                        {}
                    (-box.south west);
                \path
                    (-box.north east) --
                    node
                        [tboxstate,anchor=west,pos=-1/#1/2+\i/#1,pic actions]
                        (-box-out-\i)
                        {}
                (-box.south east);
            }
            
            \foreach \i/\j/\d in {#2}
            {
                \draw
                    [   
                        tboxarrow,
                        decoration =
                        {
                            markings,
                            mark=
                                at position 1 with
                                {
                                    \arrow[scale=1,>=triangle 45]{>}
                                }
                        }
                        ,
                        postaction={decorate}
                    ]
                    (-box-in-\i.east)
                    --
                    node
                        [pos=.8,\d]
                        {}
                    (-box-out-\j.west);
            }
        }
    },
    tbox color/.style={
        tboxstate/.append style={fill=#1},
        tboxoutline/.append style={draw=#1},
        tboxarrow/.append style={draw=#1},
    },
    trans/.style =
    {
        thick,
    },
    dot/.style =
    {
        circle,
        draw,
        minimum size=6pt,
        inner sep=0pt,
        fill,
    },
}

